LLM meets Vision-Language Models for Zero-Shot One-Class Classification

We consider the problem of zero-shot one-class visual classification, extending traditional one-class classification to scenarios where only the label of the target class is available. This method aims to discriminate between positive and negative query samples without requiring examples from the target class. We propose a two-step solution that first queries large language models for visually confusing objects and then relies on vision-language pre-trained models (e.g., CLIP) to perform classification. By adapting large-scale vision benchmarks, we demonstrate the ability of the proposed method to outperform adapted off-the-shelf alternatives in this setting. Namely, we propose a realistic benchmark where negative query samples are drawn from the same original dataset as positive ones, including a granularity-controlled version of iNaturalist, where negative samples are at a fixed distance in the taxonomy tree from the positive ones. To our knowledge, we are the first to demonstrate the ability to discriminate a single category from other semantically related ones using only its label.

==> figures/pipeline.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,464); %set diagram left start at 0, and has height of 464

%Straight Lines [id:da7461275130533311] 
\draw    (213,123) -- (287,122.51) ;
\draw [shift={(289,122.5)}, rotate = 179.62] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da9775340972657971] 
\draw    (213,328) -- (287,327.51) ;
\draw [shift={(289,327.5)}, rotate = 179.62] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Rounded Rect [id:dp8988913497105788] 
\draw  [color={rgb, 255:red, 184; green, 255; blue, 255 }  ,draw opacity=1 ][fill={rgb, 255:red, 184; green, 255; blue, 255 }  ,fill opacity=0.68 ] (303,112) .. controls (303,107.58) and (306.58,104) .. (311,104) -- (365,104) .. controls (369.42,104) and (373,107.58) .. (373,112) -- (373,136) .. controls (373,140.42) and (369.42,144) .. (365,144) -- (311,144) .. controls (306.58,144) and (303,140.42) .. (303,136) -- cycle ;
%Straight Lines [id:da06626491412631319] 
\draw    (336,254.5) -- (335.68,300.33) ;
\draw [shift={(335.67,302.33)}, rotate = 270.4] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da7764324947803993] 
\draw    (383,123) -- (417,122.53) ;
\draw [shift={(419,122.5)}, rotate = 179.2] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da2626091066907532] 
\draw    (383,328) -- (417,327.53) ;
\draw [shift={(419,327.5)}, rotate = 179.2] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da15494083094225752] 
\draw    (189,79.5) -- (418,78.51) ;
\draw [shift={(420,78.5)}, rotate = 179.75] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da6873053386226016] 
\draw    (189,79.5) -- (189,106.5) ;
%Straight Lines [id:da29455587744045797] 
\draw    (189,286.5) -- (189,313.5) ;
%Straight Lines [id:da5949313055770769] 
\draw    (509,123) -- (543,122.53) ;
\draw [shift={(545,122.5)}, rotate = 179.2] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da6163346699901688] 
\draw    (509,302) -- (543,301.53) ;
\draw [shift={(545,301.5)}, rotate = 179.2] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Rounded Rect [id:dp876294157294188] 
\draw  [color={rgb, 255:red, 184; green, 255; blue, 255 }  ,draw opacity=1 ][fill={rgb, 255:red, 184; green, 255; blue, 255 }  ,fill opacity=0.68 ] (551,112) .. controls (551,107.58) and (554.58,104) .. (559,104) -- (613,104) .. controls (617.42,104) and (621,107.58) .. (621,112) -- (621,136) .. controls (621,140.42) and (617.42,144) .. (613,144) -- (559,144) .. controls (554.58,144) and (551,140.42) .. (551,136) -- cycle ;
%Rounded Rect [id:dp10350230815292538] 
\draw  [color={rgb, 255:red, 184; green, 255; blue, 255 }  ,draw opacity=1 ][fill={rgb, 255:red, 184; green, 255; blue, 255 }  ,fill opacity=0.68 ] (551,291) .. controls (551,286.58) and (554.58,283) .. (559,283) -- (613,283) .. controls (617.42,283) and (621,286.58) .. (621,291) -- (621,315) .. controls (621,319.42) and (617.42,323) .. (613,323) -- (559,323) .. controls (554.58,323) and (551,319.42) .. (551,315) -- cycle ;
%Image [id:dp5900953604204731] 
\draw (862.48,122.92) node  {\includegraphics[width=40.72pt,height=36.38pt]{image.png}};
%Image [id:dp3642450312363963] 
\draw (862.5,171.42) node  {\includegraphics[width=40.75pt,height=36.38pt]{image.png}};
%Image [id:dp40212436619673464] 
\draw (862.5,74.42) node  {\includegraphics[width=40.75pt,height=36.37pt]{zebra_finch.jpg}};
%Shape: Rectangle [id:dp06572576483092307] 
\draw  [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=0.58 ][fill={rgb, 255:red, 255; green, 0; blue, 0 }  ,fill opacity=0.58 ] (678,56.33) -- (819.67,56.33) -- (819.67,190.33) -- (678,190.33) -- cycle ;
%Shape: Rectangle [id:dp3819209370366563] 
\draw  [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=0.58 ][fill={rgb, 255:red, 255; green, 0; blue, 0 }  ,fill opacity=0.58 ] (678,235.33) -- (819.67,235.33) -- (819.67,369.33) -- (678,369.33) -- cycle ;
%Shape: Ellipse [id:dp9801522823539239] 
\draw  [color={rgb, 255:red, 29; green, 254; blue, 42 }  ,draw opacity=1 ][fill={rgb, 255:red, 198; green, 255; blue, 203 }  ,fill opacity=1 ] (720,123.33) .. controls (720,112.01) and (732.91,102.83) .. (748.83,102.83) .. controls (764.76,102.83) and (777.67,112.01) .. (777.67,123.33) .. controls (777.67,134.66) and (764.76,143.83) .. (748.83,143.83) .. controls (732.91,143.83) and (720,134.66) .. (720,123.33) -- cycle ;
%Shape: Ellipse [id:dp5443721865194187] 
\draw  [color={rgb, 255:red, 29; green, 254; blue, 42 }  ,draw opacity=1 ][fill={rgb, 255:red, 198; green, 255; blue, 203 }  ,fill opacity=1 ] (696,302.33) .. controls (696,275.98) and (719.65,254.63) .. (748.83,254.63) .. controls (778.01,254.63) and (801.67,275.98) .. (801.67,302.33) .. controls (801.67,328.68) and (778.01,350.04) .. (748.83,350.04) .. controls (719.65,350.04) and (696,328.68) .. (696,302.33) -- cycle ;
%Image [id:dp023304743420119678] 
\draw (740.17,116) node  {\includegraphics[width=13pt,height=10pt]{zebra_finch.jpg}};
%Image [id:dp6215591469142314] 
\draw (720.92,152.08) node  {\includegraphics[width=16.13pt,height=14.63pt]{image.png}};
%Image [id:dp013155501297430483] 
\draw (794,171.33) node  {\includegraphics[width=13.5pt,height=12.5pt]{image.png}};
%Image [id:dp9609525130744843] 
\draw (794,352.33) node  {\includegraphics[width=13.5pt,height=12.5pt]{image.png}};
%Image [id:dp1617188958085607] 
\draw (718.28,323.42) node  {\includegraphics[width=12.13pt,height=11.12pt]{image.png}};
%Image [id:dp4740317117776782] 
\draw (740.17,287) node  {\includegraphics[width=13pt,height=10pt]{zebra_finch.jpg}};
%Image [id:dp0187822824642101] 
\draw (862.15,302.42) node  {\includegraphics[width=40.72pt,height=36.38pt]{image.png}};
%Image [id:dp9410809744100086] 
\draw (862.17,350.92) node  {\includegraphics[width=40.75pt,height=36.38pt]{image.png}};
%Image [id:dp455139816098761] 
\draw (862.17,253.92) node  {\includegraphics[width=40.75pt,height=36.38pt]{zebra_finch.jpg}};
%Straight Lines [id:da25102945096935625] 
\draw    (835,75.75) -- (750.7,108.61) ;
\draw [shift={(748.83,109.33)}, rotate = 338.71] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da45193992601360766] 
\draw    (836,125.25) -- (733.64,142.01) ;
\draw [shift={(731.67,142.33)}, rotate = 350.7] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da5785530744935552] 
\draw    (835.17,172) -- (803.83,172) ;
\draw [shift={(801.83,172)}, rotate = 360] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da27812010991910463] 
\draw    (836.33,353.33) -- (805,353.33) ;
\draw [shift={(803,353.33)}, rotate = 360] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da7676370199888327] 
\draw    (835,306) -- (728.36,315.82) ;
\draw [shift={(726.37,316)}, rotate = 354.74] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da9369639911319385] 
\draw    (834,256.25) -- (750.76,279.79) ;
\draw [shift={(748.83,280.33)}, rotate = 344.21] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Image [id:dp29408831074966746] 
\draw (305,104.13) node  {\includegraphics[width=15.75pt,height=16.31pt]{image.png}};
%Rounded Rect [id:dp2738997729290482] 
\draw  [color={rgb, 255:red, 184; green, 255; blue, 255 }  ,draw opacity=1 ][fill={rgb, 255:red, 184; green, 255; blue, 255 }  ,fill opacity=0.68 ] (303,317) .. controls (303,312.58) and (306.58,309) .. (311,309) -- (365,309) .. controls (369.42,309) and (373,312.58) .. (373,317) -- (373,341) .. controls (373,345.42) and (369.42,349) .. (365,349) -- (311,349) .. controls (306.58,349) and (303,345.42) .. (303,341) -- cycle ;
%Image [id:dp10434965493092974] 
\draw (305,311.13) node  {\includegraphics[width=15.75pt,height=16.31pt]{image.png}};
%Rounded Rect [id:dp8429369993751221] 
\draw  [fill={rgb, 255:red, 184; green, 255; blue, 255 }  ,fill opacity=0.68 ] (424.33,65.2) .. controls (424.33,56.25) and (431.59,49) .. (440.53,49) -- (489.13,49) .. controls (498.08,49) and (505.33,56.25) .. (505.33,65.2) -- (505.33,142.8) .. controls (505.33,151.75) and (498.08,159) .. (489.13,159) -- (440.53,159) .. controls (431.59,159) and (424.33,151.75) .. (424.33,142.8) -- cycle ;
%Straight Lines [id:da007381221474110022] 
\draw    (424.33,65.2) -- (505.33,65.2) ;
%Rounded Rect [id:dp5061875646617706] 
\draw  [fill={rgb, 255:red, 184; green, 255; blue, 255 }  ,fill opacity=0.68 ] (424.3,271.2) .. controls (424.3,262.25) and (431.55,255) .. (440.5,255) -- (489.1,255) .. controls (498.05,255) and (505.3,262.25) .. (505.3,271.2) -- (505.3,348.8) .. controls (505.3,357.75) and (498.05,365) .. (489.1,365) -- (440.5,365) .. controls (431.55,365) and (424.3,357.75) .. (424.3,348.8) -- cycle ;
%Straight Lines [id:da9839204179861565] 
\draw    (425,271.2) -- (506,271.2) ;
%Rounded Same Side Corner Rect [id:dp5393759770904907] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (505.33,142.8) .. controls (505.33,151.75) and (498.08,159) .. (489.13,159) -- (440.53,159) .. controls (431.59,159) and (424.33,151.75) .. (424.33,142.8) -- (424.33,65.2) .. controls (424.33,65.2) and (424.33,65.2) .. (424.33,65.2) -- (505.33,65.2) .. controls (505.33,65.2) and (505.33,65.2) .. (505.33,65.2) -- cycle ;
%Rounded Same Side Corner Rect [id:dp7647210729817142] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (505.3,348.8) .. controls (505.3,357.75) and (498.05,365) .. (489.1,365) -- (440.5,365) .. controls (431.55,365) and (424.3,357.75) .. (424.3,348.8) -- (424.3,271.2) .. controls (424.3,271.2) and (424.3,271.2) .. (424.3,271.2) -- (505.3,271.2) .. controls (505.3,271.2) and (505.3,271.2) .. (505.3,271.2) -- cycle ;
%Straight Lines [id:da6474650792341603] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (828,50.25) -- (827.75,375.38) ;
%Straight Lines [id:da039393011151044544] 
\draw    (189,286.5) -- (418,285.51) ;
\draw [shift={(420,285.5)}, rotate = 179.75] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da5461044514541806] 
\draw    (335.67,199.33) -- (335.99,153.5) ;
\draw [shift={(336,151.5)}, rotate = 90.4] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da9356057276550396] 
\draw    (629,123) -- (663,122.53) ;
\draw [shift={(665,122.5)}, rotate = 179.2] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da21311396579214703] 
\draw    (629,302) -- (663,301.53) ;
\draw [shift={(665,301.5)}, rotate = 179.2] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

% Text Node
\draw (163,113.33) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\fontfamily{pcr}\selectfont \textbf{Finch}}};
% Text Node
\draw (171.67,319) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\fontfamily{pcr}\selectfont \textbf{Bird}}};
% Text Node
\draw (338,124) node   [align=left] {\begin{minipage}[lt]{30.6pt}\setlength\topsep{0pt}
{\fontfamily{pcr}\selectfont LLM}
\end{minipage}};
% Text Node
\draw (335.17,225.5) node   [align=left] {\begin{minipage}[lt]{108.12pt}\setlength\topsep{0pt}
\begin{center}
{\fontfamily{pcr}\selectfont \textit{"Generate K visually confusing objects"}}
\end{center}

\end{minipage}};
% Text Node
\draw (430.33,68.2) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\fontfamily{pcr}\selectfont \textcolor[rgb]{0.05,0.96,0.1}{+ }\textbf{\textcolor[rgb]{0.05,0.96,0.1}{Finch}}}\\{\fontfamily{pcr}\selectfont \textcolor[rgb]{1,0.1,0}{- Sparrow}}\\{\fontfamily{pcr}\selectfont \textcolor[rgb]{1,0.1,0}{- Bunting}}\\{\fontfamily{pcr}\selectfont \textcolor[rgb]{1,0.1,0}{- Lark }}};
% Text Node
\draw (427,274.2) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\fontfamily{pcr}\selectfont \textcolor[rgb]{0.05,0.96,0.1}{+ }\textbf{\textcolor[rgb]{0.05,0.96,0.1}{Bird}}}\\{\fontfamily{pcr}\selectfont \textcolor[rgb]{1,0,0}{- Bats}}\\{\fontfamily{pcr}\selectfont \textcolor[rgb]{1,0,0}{- Moths}}\\{\fontfamily{pcr}\selectfont \textcolor[rgb]{1,0,0}{- Squirrels}}\\};
% Text Node
\draw (586,124) node   [align=left] {\begin{minipage}[lt]{30.6pt}\setlength\topsep{0pt}
{\fontfamily{pcr}\selectfont CLIP}
\end{minipage}};
% Text Node
\draw (586,303) node   [align=left] {\begin{minipage}[lt]{30.6pt}\setlength\topsep{0pt}
{\fontfamily{pcr}\selectfont CLIP}
\end{minipage}};
% Text Node
\draw (149,85.75) node   [align=left] {\begin{minipage}[lt]{68pt}\setlength\topsep{0pt}
{\fontfamily{pcr}\selectfont Example a.}
\end{minipage}};
% Text Node
\draw (149,302.5) node   [align=left] {\begin{minipage}[lt]{68pt}\setlength\topsep{0pt}
{\fontfamily{pcr}\selectfont Example b.}
\end{minipage}};
% Text Node
\draw (837.33,203.17) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\fontfamily{pcr}\selectfont Queries}};
% Text Node
\draw (338,329) node   [align=left] {\begin{minipage}[lt]{30.6pt}\setlength\topsep{0pt}
{\fontfamily{pcr}\selectfont LLM}
\end{minipage}};
% Text Node
\draw (488,53.67) node   [align=left] {\begin{minipage}[lt]{68pt}\setlength\topsep{0pt}
{\fontfamily{pcr}\selectfont Classes}
\end{minipage}};
% Text Node
\draw (488,261.67) node   [align=left] {\begin{minipage}[lt]{68pt}\setlength\topsep{0pt}
{\fontfamily{pcr}\selectfont Classes}
\end{minipage}};


\end{tikzpicture}

==> plots/heatmap/heatmap.tex <==
% % This file was created with tikzplotlib v0.10.1.
% \begin{tikzpicture}

% \definecolor{darkgray176}{RGB}{176,176,176}
% \definecolor{green}{RGB}{0,128,0}
% \definecolor{lightgray204}{RGB}{204,204,204}

% \begin{axis}[
% colorbar,
% colorbar style={ylabel={}},
% colormap={mymap}{[1pt]
%   rgb(0pt)=(0,0,0.3);
%   rgb(1pt)=(0,0,1);
%   rgb(2pt)=(1,1,1);
%   rgb(3pt)=(1,0,0);
%   rgb(4pt)=(0.5,0,0)
% },
% legend cell align={left},
% legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
% point meta max=12,
% point meta min=-12,
% tick align=outside,
% tick pos=left,
% x grid style={darkgray176},
% xmin=-0.5, xmax=9.5,
% xtick style={color=black},
% y dir=reverse,
% ylabel={thresholds (lowest to highest)},
% ymin=-0.5, ymax=499.5,
% axis y line=none,
% xlabel={level},
% ]
 

% \addplot [draw=green, fill=green, mark=*, only marks]
% table{%
% x  y
% 0 1
% 1 51
% 2 137
% 3 183
% 4 237
% 5 213
% 6 280
% 7 264
% 8 304
% 9 297
% };
% \addlegendentry{Best threshold per level}

% \addplot [semithick, draw=black]
% table {%
% -1 225
% 0 225
% 1 225
% 2 225
% 3 225
% 4 225
% 5 225
% 6 225
% 7 225
% 8 225
% 9 225
% 10 225
% };
% \addlegendentry{ImageNet Threshold}

% \addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=9.5, ymin=499.5, ymax=-0.5] {plots/heatmap-000.png};

% \addplot [draw=green, fill=green, mark=*, only marks, forget plot]
% table{%
% x  y
% 0 1
% 1 51
% 2 137
% 3 183
% 4 237
% 5 213
% 6 280
% 7 264
% 8 304
% 9 297
% };
% %\addlegendentry{Best threshold per level}

% \addplot [semithick, draw=black, forget plot]
% table {%
% -1 225
% 0 225
% 1 225
% 2 225
% 3 225
% 4 225
% 5 225
% 6 225
% 7 225
% 8 225
% 9 225
% 10 225
% };
% %\addlegendentry{ImageNet Threshold}


% \end{axis}

% \end{tikzpicture}

\begin{tikzpicture}
  \begin{axis}[enlargelimits=false,colorbar,colormap/Purples]
    \addplot [matrix plot,point meta=explicit]
      coordinates {
        (0,0) [84.83] (1,0) [56.11] (2,0) [97.79] (3,0) [88.31] (4,0) [95.97] (5,0) [43.25] (6,0) [0] (7,0) [77.71]
        (0,1) [84.77] (1,1) [55.73] (2,1) [97.88] (3,1) [86.88] (4,1) [96.42] (5,1) [43.79] (6,1) [0] (7,1) [77.58]
        (0,2) [83.79] (1,2) [54.92] (2,2) [98.09] (3,2) [82.72] (4,2) [97.39] (5,2) [46.73] (6,2) [0] (7,2) [77.27]
        (0,3) [80.39] (1,3) [52.72] (2,3) [98.06] (3,3) [77.24] (4,3) [98.01] (5,3) [50.81] (6,3) [0] (7,3) [76.20]
        (0,4) [73.69] (1,4) [52.80] (2,4) [93.23] (3,4) [96.06] (4,4) [86.53] (5,4) [39.73] (6,4) [0] (7,4) [73.67]
        (0,5) [69.20] (1,5) [48.50] (2,5) [96.24] (3,5) [64.28] (4,5) [97.92] (5,5) [63.94] (6,5) [0] (7,5) [73.35]
        (0,6) [50.17] (1,6) [43.52] (2,6) [88.51] (3,6) [45.65] (4,6) [92.16] (5,6) [74.56] (6,6) [0] (7,6) [65.76]
      };
  \end{axis}
\end{tikzpicture}


==> plots/heatmap/heatmap_all_datasets2.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{green}{RGB}{0,128,0} %{255,210,0} %{0,128,0} %{128,0,128} %{246,190,0}
\definecolor{lightgray204}{RGB}{204,204,204}

\begin{axis}[
width=12cm,
height=7cm,
colorbar,
colorbar style={ylabel={}},
colormap={mymap}{[1pt]
  rgb(0pt)=(0,0,0.3);
  rgb(1pt)=(0,0,1);
  rgb(2pt)=(1,1,1);
  rgb(3pt)=(1,0,0);
  rgb(4pt)=(0.5,0,0)
},
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.03,0.03)},
  anchor=south west,
  draw=lightgray204
},
point meta max=12,
point meta min=-12,
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-0.5, xmax=19.5,
xtick style={color=black},
xtick={0,1,2,3,4,5,6,7,8,9,'',11,'',13,'',15,'',17,'',19},
xticklabel style={rotate=90.0},
xticklabels={
  iNat 0,
  iNat 1,
  iNat 2,
  iNat 3,
  iNat 4,
  iNat 5,
  iNat 6,
  iNat 7,
  iNat 8,
  iNat 9,
  ,
  Textures,
  ,
  EuroSAT,
  ,
  Food,
  ,
  Pets,
  ,
  SUN
},
y dir=reverse,
ylabel={Thresholds (lowest to highest)},
ymin=-0.5, ymax=499.5
]
\addplot [draw=green, fill=green, mark=*, only marks]
table{%
x  y
0 1
1 51
2 137
3 183
4 237
5 213
6 280
7 264
8 304
9 297
10 nan
11 224
12 nan
13 15
14 nan
15 194
16 nan
17 141
18 nan
19 359
};
\addlegendentry{Best threshold per dataset}
\addplot [semithick, draw=black]
table {%
-0.5 225
20.5 225
};
\addlegendentry{ImageNet Threshold}
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=19.5, ymin=499.5, ymax=-0.5] {plots/heatmap/heatmap_all_datasets-001.png};
\addplot [draw=green, fill=green, mark=*, only marks, mark size=3pt, forget plot]
table{%
x  y
0 1
1 51
2 137
3 183
4 237
5 213
6 280
7 264
8 304
9 297
10 nan
11 224
12 nan
13 15
14 nan
15 194
16 nan
17 141
18 nan
19 359
};
% \addlegendentry{Best threshold per dataset}
% \path [draw=black, semithick]
% (axis cs:-0.5,225)
% --(axis cs:20.5,225);
%\addlegendentry{ImageNet Threshold}

\addplot [semithick, draw=black, forget plot]
table {%
-0.5 225
20.5 225
};
\end{axis}

\end{tikzpicture}


==> plots/heatmap/heatmap_other_datasets.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{green}{RGB}{0,128,0}
\definecolor{lightgray204}{RGB}{204,204,204}

\begin{axis}[
colorbar,
colorbar style={ylabel={}},
colormap={mymap}{[1pt]
  rgb(0pt)=(0,0,0.3);
  rgb(1pt)=(0,0,1);
  rgb(2pt)=(1,1,1);
  rgb(3pt)=(1,0,0);
  rgb(4pt)=(0.5,0,0)
},
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
point meta max=12,
point meta min=-12,
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-0.5, xmax=4.5,
xtick style={color=black},
xtick={0,1,2,3,4,5},
% xticklabels={dtd,eurosat,food101,oxford_pets,sun397},
y dir=reverse,
ylabel={thresholds (lowest to highest)},
ymin=-0.5, ymax=499.5,
axis y line=none,
xlabel={Datasets},
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=4.5, ymin=499.5, ymax=-0.5] {plots/heatmapothers.png};
\addplot [draw=green, fill=green, mark=*, only marks]
table{%
x  y
0 224
1 15
2 194
3 141
4 359
};
\addlegendentry{Best threshold per dataset}
\path [draw=black, semithick]
(axis cs:-0.5,225)
--(axis cs:4.5,225);

\end{axis}

\end{tikzpicture}


==> plots/heatmap/new_heatmap.tex <==
\usepgfplotslibrary{groupplots,dateplot}
\usetikzlibrary{patterns,shapes.arrows}
\pgfplotsset{compat=newest}

\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{green}{RGB}{0,128,0}
\definecolor{lightgray204}{RGB}{204,204,204}

\begin{axis}[
width=4cm,
height=5cm,
colorbar,
colorbar style={ylabel={Relative performance}},
colormap={mymap}{[1pt]
  rgb(0pt)=(0,0,0.3);
  rgb(1pt)=(0,0,1);
  rgb(2pt)=(1,1,1);
  rgb(3pt)=(1,0,0);
  rgb(4pt)=(0.5,0,0)
},
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.03,0.03)},
  anchor=south west,
  draw=lightgray204
},
point meta max=12,
point meta min=-12,
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-0.5, xmax=21.55,
xtick style={color=black},
xtick={0,1,2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17,18,19},
xticklabel style={rotate=90.0},
xticklabels={
  iNat 0,
  iNat 1,
  iNat 2,
  iNat 3,
  iNat 4,
  iNat 5,
  iNat 6,
  iNat 7,
  iNat 8,
  iNat 9,
  ,
  SUN,
  ,
  Food,
  ,
  Textures,
  ,
  Pets,
  ,
  EuroSAT
},
y dir=reverse,
ylabel={thresholds (lowest to highest)},
ymin=-0.5, ymax=499.5
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=19.5, ymin=499.5, ymax=-0.5] {plots/heatmap/heatmap_all_datasets-005.png};
\addplot [draw=green, fill=green, mark=*, only marks]
table{%
x  y
0 1
1 51
2 137
3 183
4 237
5 213
6 280
7 264
8 304
9 297
10 nan
11 359
12 nan
13 194
14 nan
15 224
16 nan
17 141
18 nan
19 15
};
\addlegendentry{Best threshold per dataset}
\path [draw=black, semithick]
(axis cs:-0.5,225)
--(axis cs:20.5,225);

\end{axis}

\end{tikzpicture}


==> plots/query_distance/varyQdistanceOpenclip.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{green}{RGB}{0,128,0}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{pink}{RGB}{255,192,203}

\begin{axis}[
legend cell align={left},
legend style={
width=7cm, 
height=7cm,
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.03,0.97)},
  anchor=north west,
  draw=lightgray204
},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={Distance},
xmajorgrids,
xmin=0.7, xmax=7.3,
xtick style={color=black},
y grid style={darkgray176},
ylabel={macro F1 score (\%)},
ymajorgrids,
ymin=37.508022967026, ymax=94.7572976574801,
ytick style={color=black}
]
\path [draw=pink, fill=pink, opacity=0.5]
(axis cs:1,48.4433065023201)
--(axis cs:1,46.4281268096107)
--(axis cs:2,57.5721805731887)
--(axis cs:3,66.607828651548)
--(axis cs:4,73.825955004737)
--(axis cs:5,79.4846353899053)
--(axis cs:6,82.7432412162099)
--(axis cs:7,85.9773665868694)
--(axis cs:7,88.3585423371635)
--(axis cs:7,88.3585423371635)
--(axis cs:6,85.3106473933927)
--(axis cs:5,82.0348381085758)
--(axis cs:4,76.5431038279832)
--(axis cs:3,69.35963433973)
--(axis cs:2,60.221378808284)
--(axis cs:1,48.4433065023201)
--cycle;

\path [draw=green, fill=green, opacity=0.5]
(axis cs:1,41.5803300316299)
--(axis cs:1,40.110262725683)
--(axis cs:2,50.3727455029446)
--(axis cs:3,60.8804940030865)
--(axis cs:4,70.8256139123201)
--(axis cs:5,78.7742498969755)
--(axis cs:6,85.7154757112723)
--(axis cs:7,90.5092676020079)
--(axis cs:7,92.1550578988231)
--(axis cs:7,92.1550578988231)
--(axis cs:6,87.7624623329525)
--(axis cs:5,81.3075941123228)
--(axis cs:4,73.5633602962647)
--(axis cs:3,63.6670447141004)
--(axis cs:2,52.8012016598583)
--(axis cs:1,41.5803300316299)
--cycle;

\addplot [semithick, pink, mark=*, mark size=3, mark options={solid}]
table {%
1 47.4357166559654
2 58.8967796907364
3 67.983731495639
4 75.1845294163601
5 80.7597367492405
6 84.0269443048013
7 87.1679544620165
};
\addlegendentry{ANP+MT}
\addplot [semithick, green, mark=*, mark size=3, mark options={solid}]
table {%
1 40.8452963786564
2 51.5869735814015
3 62.2737693585934
4 72.1944871042924
5 80.0409220046492
6 86.7389690221124
7 91.3321627504155
};
\addlegendentry{MT}
\end{axis}

\end{tikzpicture}


==> plots/query_distance/varyQdistanceVITB.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{green}{RGB}{0,128,0}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{pink}{RGB}{255,192,203}

\begin{axis}[
legend cell align={left},
legend style={
width=7cm, 
height=7cm,
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.03,0.97)},
  anchor=north west,
  draw=lightgray204
},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={Distance},
xmajorgrids,
xmin=0.7, xmax=7.3,
xtick style={color=black},
y grid style={darkgray176},
ylabel={macro F1 score (\%)},
ymajorgrids,
ymin=37.508022967026, ymax=94.7572976574801,
ytick style={color=black}
]
\path [draw=pink, fill=pink, opacity=0.5]
(axis cs:1,48.4433065023201)
--(axis cs:1,46.4281268096107)
--(axis cs:2,57.5721805731887)
--(axis cs:3,66.607828651548)
--(axis cs:4,73.825955004737)
--(axis cs:5,79.4846353899053)
--(axis cs:6,82.7432412162099)
--(axis cs:7,85.9773665868694)
--(axis cs:7,88.3585423371635)
--(axis cs:7,88.3585423371635)
--(axis cs:6,85.3106473933927)
--(axis cs:5,82.0348381085758)
--(axis cs:4,76.5431038279832)
--(axis cs:3,69.35963433973)
--(axis cs:2,60.221378808284)
--(axis cs:1,48.4433065023201)
--cycle;

\path [draw=green, fill=green, opacity=0.5]
(axis cs:1,41.5803300316299)
--(axis cs:1,40.110262725683)
--(axis cs:2,50.3727455029446)
--(axis cs:3,60.8804940030865)
--(axis cs:4,70.8256139123201)
--(axis cs:5,78.7742498969755)
--(axis cs:6,85.7154757112723)
--(axis cs:7,90.5092676020079)
--(axis cs:7,92.1550578988231)
--(axis cs:7,92.1550578988231)
--(axis cs:6,87.7624623329525)
--(axis cs:5,81.3075941123228)
--(axis cs:4,73.5633602962647)
--(axis cs:3,63.6670447141004)
--(axis cs:2,52.8012016598583)
--(axis cs:1,41.5803300316299)
--cycle;

\addplot [semithick, pink, mark=*, mark size=3, mark options={solid}]
table {%
1 47.4357166559654
2 58.8967796907364
3 67.983731495639
4 75.1845294163601
5 80.7597367492405
6 84.0269443048013
7 87.1679544620165
};
\addlegendentry{ANP+MT}
\addplot [semithick, green, mark=*, mark size=3, mark options={solid}]
table {%
1 40.8452963786564
2 51.5869735814015
3 62.2737693585934
4 72.1944871042924
5 80.0409220046492
6 86.7389690221124
7 91.3321627504155
};
\addlegendentry{MT}
\end{axis}

\end{tikzpicture}


==> sections/introduction2.tex <==
\section{Introduction}
\label{sec:intro}

% motivate one class classification 
% motivate zero shot one class classification 
% explain different to OOD detection, Image Retrieval and to one class vs all
% explain the challenge of zero shot one class (estimating boundaries)
% overview of method to solve it 
% overview of results 

Recently, the literature has shown the feasibility of classifying visual objects in a zero-shot fashion, where only class labels (or a textual description) are leveraged to infer a classifier on images~\cite{clip,zeroshot}. These approaches make use of vision-language pre-trained models such as CLIP~\cite{clip} that align text and images, showing good performance in datasets containing from ten to hundreds of classes~\cite{coop,multimodality}. Such models allow to perform open-vocabulary classification, where the set of objects to classify is not limited to the training dataset. These approaches have been since extended to multiple applications such as few-shot classification~\cite{coop}, image segmentation~\cite{clipseg} and 3D reconstruction~\cite{clip3d}. 

In this paper, we are interested in the limit case of identifying a single category (\emph{i.e.}, one-class classification), where the goal is to obtain a discriminator for a single class~\cite{deeponeclass}. One-class classification has been extensively studied as it encapsulates multiple research fields~\cite{oneclasssurvey,oneclasssvm,oneclasssemi} including the well-known problem of anomaly detection where the aim is to identify outliers (\emph{i.e.}, points that do not belong to the target class) and finds its utility in various domains such as fraud detection, healthcare and damage detection. Another practical application to one-class classification is wake-word detection in edge devices where the goal is to detect a certain signal that triggers some action from the system. 

While one-class classification has received considerable attention, existing methods require gathering training samples to train a one-class classifier for a specific application and are by construction not flexible to new concepts. In this work, we are interested in expanding this setting to encompass the open-vocabulary case, namely zero-shot one-class classification, which allows for easy adaptation to different target classes. This finds its utility in multiple industrial use-cases where collecting training data on the ``special'' class is expensive or in robotic systems that require the capability for flexible adjustment in object detection. Despite the importance of such a setting, literature lacks direct references to this task.

Having introduced the framework for zero-shot one-class classification, it is pertinent to contrast it with classical Image-Text retrieval tasks, which operate under different assumptions. In classical Image-Text retrieval, the user leverages a large database of query images to retrieve the top-K queries based on a predefined similarity score~\cite{textimageretrieval1, textimageretrieval2}. Such a methodology relies on an extensive offline database, which contrasts with the online nature of zero-shot one-class classification. As illustrated in Figure~\ref{fig:main}, in our framework, each query is processed individually and is not part of an existing database, focusing solely on determining if a single image belongs to the target class. This capability is particularly advantageous in scenarios such as robotic devices, where the classification needs can change in real-time. %Furthermore, while some instance retrieval tasks incorporate a binary classification mechanism trained on text labels, these systems typically do not support the open-vocabulary case~\cite{textimageretrieval2}. 

Interestingly, existing zero-shot classification approaches are not easily adapted to this limit case. Since they typically require multiple categories to build their classifiers, such a set of all possible categories at test time is often not available. While classifying multiple objects typically involves estimating the boundaries between classes, one-class classification requires defining these boundaries solely based on examples from the class in question. Recent works also consider the case of zero-shot out of distribution~\cite{mcm,clipn,zoc}, mainly reporting AUC scores where the exact boundary estimation, through the use of an explicit threshold, is not directly addressed. However, we argue that validation samples are not necessarily available in practice, particularly in zero-shot classification, and that the question of finding the absolute position of the boundary still holds untapped potential.

Estimating the boundary of each class would require either collecting training samples or defining the set of all possible negative classes which in practice is intractable. We instead elaborate a simple, yet very effective solution, by collecting a set of high quality negative labels to define the boundary of the class. Such a set is constructed by prompting a Large Language Model (LLM) for the most visually confusing objects, as depicted in Figure~\ref{fig:intro}. This allows to construct a corpus of negative-labels adapted for target task. We further regularize this decision boundary using a transferred threshold in order to restrain the positive samples. Additionally, we run extensive experiments to validate our methodology against adapted off-the-shelf baselines and show its robustness on multiple settings including a granularity-controlled version of iNaturalist. Our contributions are as follows:

\begin{figure}[t!]
    \centering
        \includegraphics[width=1\textwidth]{figures/mainfig_decisionboundaries.png}
    \caption{In the zero-shot one-class classification problem, the class is defined using a prompt text, and the task is to accept or reject query images independently. As the prompt text varies, the decision boundaries of the class also varies. Such a task is challenging as it requires an accurate estimate of the boundaries of each class.}
    \label{fig:main}
\end{figure}

\begin{enumerate}
\item To the best of our knowledge, we are the first to tackle the problem of zero-shot one-class classification, where only the label of the class of interest is available;
\item We propose a realistic benchmark where negative query samples are drawn from the same original dataset as positive ones. We include a granularity-controlled version of iNaturalist, where negative samples are at a fixed distance in the taxonomy tree from the positive ones;
\item We propose a methodology making use of an LLM and a vision-language pre-trained model. We conduct extensive experiments to demonstrate the robustness of our approach across a diverse range of tasks, showing its benefits compared to adapted off-the-shelf alternatives.
\end{enumerate}

==> tables/FT_selection.tex <==
\renewcommand{\arraystretch}{1.2}

\begin{table}[h!]
  \caption{Average macro F1 score for multiple datasets. Comparison for selecting the threshold from ImageNet1K.
  }
   \label{tab:ft_selection}
  \centering
  \resizebox{\textwidth}{!}{\begin{tabular}{@{}c|c|c|c|c|c|c|c@{}}
    \toprule % cmidrule(r){2-5}
Selection criteria &	iNat	& SUN	& Food	& Textures	& Pets & EuroSAT	& Average \\
\cline{1-8}
\parbox{4cm}{\centering Hyperparameter search\\} &$54.70\pm1.18$&$96.63\pm0.20$&$95.41\pm0.21$&$82.42\pm0.67$&$84.16\pm0.38$&$\mathbf{75.82\pm0.97}$&$81.53$\\

\hline
 \parbox{4cm}{\centering Average of optimal thresholds}	&$\mathbf{56.60\pm1.25}$&$\mathbf{97.36\pm0.21}$&$\mathbf{97.49\pm0.13}$&$\mathbf{86.62\pm0.71}$&$\mathbf{91.56\pm0.27}$&$72.48\pm1.07$&$\mathbf{83.68}$\\
\bottomrule
\end{tabular}}
\end{table}


==> tables/main_results_all.tex <==
\renewcommand{\arraystretch}{1.2}

\begin{table}
  \caption{Average macro F1 score for multiple datasets. Our methods are in bold.
  }
   \label{tab:main_performance}
  \centering
  \scalebox{0.67}{\begin{tabular}{@{}c|c|c|c|c|c|c|c||c@{}}
    \toprule % cmidrule(r){2-5}
Backbone & Method &	iNat	& SUN	& Food	& Textures	& Pets & EuroSAT	& Average \\
\cline{1-9}
\multirow{5}{*}{\parbox{2cm}{\centering ViT-B-16 CLIP}} & CLIPN~\cite{clipn}	&	$41.95\pm0.79$ &	$85.66\pm0.47$ &$69.86\pm0.77$&	$52.28\pm0.67$&	$73.84\pm0.76$&	$60.67\pm0.90$&	$64.05$ \\
& \textbf{ANP}	 &$55.81\pm1.05$&$85.41\pm0.78$&$86.85\pm0.57$&$66.88\pm1.30$&$54.90\pm1.26$&$52.79\pm1.17$&$67.10$\\
& \textbf{FT}	&$54.32\pm1.10$&$95.14\pm0.30$&$95.31\pm0.17$&$\mathbf{78.51\pm0.89}$&$90.24\pm0.77$&$70.32\pm0.88$&$80.63$\\
& CLIPN\cite{clipn} + \textbf{FT}	&$50.77\pm1.11$&$\mathbf{96.59\pm0.16}$&$92.18\pm0.31$&$76.70\pm0.79$&$89.50\pm0.52$&$\mathbf{72.03\pm1.21}$&$79.62$\\
&\textbf{ANP+FT}  &$\mathbf{60.64\pm1.02}$&$94.35\pm0.36$&$\mathbf{95.62\pm0.17}$&$77.24\pm1.09$&$\mathbf{93.46\pm0.81}$&$65.95\pm0.91$&$\mathbf{81.20}$\\
\hline
\multirow{5}{*}{\parbox{2cm}{\centering ViT-B-32 CLIP}} 
& ZOC\cite{zoc}	&$55.05\pm0.99$&$93.61\pm0.32$&$92.18\pm0.24$&$73.88\pm0.66$&$88.53\pm0.77$&${65.38\pm1.14}$&$78.16$\\
& \textbf{ANP}	&$54.44\pm0.97$&$86.32\pm0.71$&$83.54\pm0.68$&$69.38\pm1.12$&$55.14\pm1.38$&$48.36\pm1.20$&$66.20$\\
& \textbf{FT}	&$54.26\pm1.03$&$94.68\pm0.28$&$93.82\pm0.21$&$77.06\pm0.68$&$87.61\pm0.76$&$\mathbf{65.70\pm0.83}$&$78.85$\\
& ZOC\cite{zoc}+\textbf{FT}	&$53.78\pm0.10$&$\mathbf{95.30\pm0.28}$&$93.74\pm0.21$&${77.51\pm0.68}$&$87.91\pm0.76$&$64.82\pm1.05$&$78.43$\\
&\textbf{ANP+FT} &$\mathbf{60.32\pm0.99}$&$94.19\pm0.38$&$\mathbf{94.18\pm0.20}$&$\mathbf{78.21\pm0.88}$&$\mathbf{90.97\pm0.88}$&$59.72\pm0.98$&$\mathbf{79.60}$\\
\hline
\multirow{3}{*}{\parbox{2cm}{\centering ViT-H-14 OpenCLIP}} & \textbf{ANP}	&$60.14{\scriptsize\pm1.17}$&	${90.98{\scriptsize\pm0.58}}$&	$91.90{\scriptsize\pm0.5}$&	$81.00{\scriptsize\pm0.94}$&	$73.33{\scriptsize\pm1.39}$&	$49.12{\scriptsize\pm1.17}$&	
$74.42$ \\
& \textbf{FT}&	$56.10{\scriptsize\pm1.21}$&	$88.30{\scriptsize\pm0.66}$&	$97.78{\scriptsize\pm0.11}$&	$84.83{\scriptsize\pm0.50}$&	$95.96{\scriptsize\pm0.16}$&	$43.25{\scriptsize\pm0.51}$&	$77.71$ \\
& \textbf{ANP+FT}	&$\mathbf{64.08{\scriptsize\pm1.12}}$&	$\mathbf{94.06{\scriptsize\pm0.48}}$&	$\mathbf{97.83{\scriptsize\pm0.11}}$&	$\mathbf{87.09{\scriptsize\pm0.61}}$&	$\mathbf{98.15{\scriptsize\pm0.12}}$&	$\mathbf{60.74{\scriptsize\pm0.67}}$&	$\mathbf{83.66}$ \\
\bottomrule
\end{tabular}}
\end{table}


% & \textbf{FT}&	$56.10{\scriptsize\pm1.21}$&	$88.30{\scriptsize\pm0.66}$&	$97.78{\scriptsize\pm0.11}$&	$84.83{\scriptsize\pm0.50}$&	$95.96{\scriptsize\pm0.16}$&	$43.25{\scriptsize\pm0.51}$&	$77.71$ \\
% & \textbf{ANP+FT}	&$\mathbf{64.08{\scriptsize\pm1.12}}$&	$\mathbf{94.06{\scriptsize\pm0.48}}$&	$\mathbf{97.83{\scriptsize\pm0.11}}$&	$\mathbf{87.09{\scriptsize\pm0.61}}$&	$\mathbf{98.15{\scriptsize\pm0.12}}$&	$\mathbf{60.74{\scriptsize\pm0.67}}$&	$\mathbf{83.66}$ \\


% \renewcommand{\arraystretch}{1.2}

% \begin{table}
%   \caption{Average macro F1 score for multiple datasets. Our methods are in bold.
%   }
%    \label{tab:main_performance}
%   \centering
%   \scalebox{0.67}{\begin{tabular}{@{}c|c|c|c|c|c|c|c||c@{}}
%     \toprule % cmidrule(r){2-5}
% Backbone & Method &	iNat	& SUN	& Food	& Textures	& Pets & EuroSAT	& Average \\
% \cline{1-9}
% \multirow{2}{*}{\parbox{2cm}{\centering ViT-B-16 CLIP}} & CLIPN~\cite{clipn}	&	$41.95\pm0.79$ &	$85.66\pm0.47$ &$69.86\pm0.77$&	$52.28\pm0.67$&	$73.84\pm0.76$&	$60.67\pm0.90$&	$64.05$ \\
% &\textbf{ANP+FT} (ours) &$\mathbf{60.64\pm1.02}$&$94.35\pm0.36$&$\mathbf{95.62\pm0.17}$&$77.24\pm1.09$&$\mathbf{93.46\pm0.81}$&$65.95\pm0.91$&$\mathbf{81.20}$\\
% \hline
% \multirow{2}{*}{\parbox{2cm}{\centering ViT-B-32 CLIP}} 
% & ZOC\cite{zoc}	&$55.05\pm0.99$&$93.61\pm0.32$&$92.18\pm0.24$&$73.88\pm0.66$&$88.53\pm0.77$&${65.38\pm1.14}$&$78.11$\\
% &\textbf{ANP+FT} (ours) &$\mathbf{60.32\pm0.99}$&$94.19\pm0.38$&$\mathbf{94.18\pm0.20}$&$\mathbf{78.21\pm0.88}$&$\mathbf{90.97\pm0.88}$&$59.72\pm0.98$&$\mathbf{79.60}$\\
% \hline
% OpenCLIP& \textbf{ANP+FT} (ours)	&${64.08{\scriptsize\pm1.12}}$&	${94.06{\scriptsize\pm0.48}}$&	${97.83{\scriptsize\pm0.11}}$&	${87.09{\scriptsize\pm0.61}}$&	${98.15{\scriptsize\pm0.12}}$&	${60.74{\scriptsize\pm0.67}}$&	${83.66}$ \\
% \bottomrule
% \end{tabular}}
% \end{table}

==> tables/main_results_old.tex <==
% \begin{table}
%   \caption{Average macro-F1-score for multiple datasets.
%   }
%    \label{tab:main_performance}
%   \centering
%   \scalebox{0.75}{\begin{tabular}{@{}c|c|c|c|c|c|c|c|c@{}}
%     \hline % cmidrule(r){2-5}
% Backbone & Method &	iNat	& SUN	& Food	& Textures	& Pets & EuroSAT	& Average \\
% \cline{1-9}
% \multirow{3}{*}{\parbox{2cm}{\centering ViT-B-16 CLIP}} & CLIPN~\cite{clipn}	&	$37.94{\scriptsize\pm0.46}$ &	$90.49{\scriptsize\pm0.29}$ &$52.92{\scriptsize\pm0.76}$&	$45.88{\scriptsize\pm0.51}$&	$61.96{\scriptsize\pm0.82}$&	$35.06{\scriptsize\pm0.22}$&	$54.04{\scriptsize\pm0.51}$ \\
% & FT	&	$54.39{\scriptsize\pm1.02}$ &	$89.17{\scriptsize\pm0.60}$ &$94.16{\scriptsize\pm0.19}$&	$73.15{\scriptsize\pm1.01}$&	$91.80{\scriptsize\pm0.39}$&	$42.19{\scriptsize\pm0.32}$&	$74.14{\scriptsize\pm0.59}$ \\
% & ANP+FT &	$\mathbf{60.82{\scriptsize\pm1.04}}$ &	$\mathbf{93.20{\scriptsize\pm0.48}}$ &	$\mathbf{95.76{\scriptsize\pm0.16}}$&	$\mathbf{73.86{\scriptsize\pm1.23}}$&	$\mathbf{92.21{\scriptsize\pm1.03}}$&	$\mathbf{54.50{\scriptsize\pm0.44}}$&	$\mathbf{78.39{\scriptsize\pm0.73}}$ \\
% \hline
% \multirow{2}{*}{\parbox{2cm}{\centering ViT-H-14 Open-CLIP}}  & FT&	$56.10{\scriptsize\pm1.21}$&	$88.30{\scriptsize\pm0.66}$&	$97.78{\scriptsize\pm0.11}$&	$84.83{\scriptsize\pm0.50}$&	$95.96{\scriptsize\pm0.16}$&	$43.25{\scriptsize\pm0.51}$&	$77.71{\scriptsize\pm0.53}$ \\
% & ANP+FT	&$\mathbf{64.08{\scriptsize\pm1.12}}$&	$\mathbf{94.06{\scriptsize\pm0.48}}$&	$\mathbf{97.83{\scriptsize\pm0.11}}$&	$\mathbf{87.09{\scriptsize\pm0.61}}$&	$\mathbf{98.15{\scriptsize\pm0.12}}$&	$\mathbf{60.74{\scriptsize\pm0.67}}$&	$\mathbf{83.66{\scriptsize\pm0.52}}$ \\
% \hline
% \end{tabular}}
 
% \end{table}
\renewcommand{\arraystretch}{1.2}

\begin{table}
  \caption{Average macro F1 score for multiple datasets. The second-best score is underlined when confidence intervals intersect. Our methods are in bold.
  }
   \label{tab:main_performance}
  \centering
  \scalebox{0.7}{\begin{tabular}{@{}c|c|c|c|c|c|c|c|c@{}}
    \toprule % cmidrule(r){2-5}
Backbone & Method &	iNat	& SUN	& Food	& Textures	& Pets & EuroSAT	& Average \\
\cline{1-9}
\multirow{4}{*}{\parbox{2cm}{\centering ViT-B-16 CLIP}} & CLIPN~\cite{clipn}	&	$37.94{\scriptsize\pm0.46}$ &	$90.49{\scriptsize\pm0.29}$ &$52.92{\scriptsize\pm0.76}$&	$45.88{\scriptsize\pm0.51}$&	$61.96{\scriptsize\pm0.82}$&	$35.06{\scriptsize\pm0.22}$&	$54.04{\scriptsize\pm0.51}$ \\
& ZOC\cite{zoc}	&	$$ &	$$ &$$&	$$&	$$&	$$&	$2$  \\
& \textbf{ANP}	&	$$ &	$$ &$$&	$$&	$$&	$$&	$2$  \\
& \textbf{FT}	&	$54.39{\scriptsize\pm1.02}$ &	$89.17{\scriptsize\pm0.60}$ &$94.16{\scriptsize\pm0.19}$&	$\underline{73.15{\scriptsize\pm1.01}}$&	$\underline{91.80{\scriptsize\pm0.39}}$&	$42.19{\scriptsize\pm0.32}$&	$74.14{\scriptsize\pm0.59}$ \\
& CLIPN\cite{clipn} + \textbf{FT}	&	$50.16{\scriptsize\pm1.10}$ &	$\mathbf{95.11{\scriptsize\pm0.32}}$ &$86.22{\scriptsize\pm0.43}$&	${70.39{\scriptsize\pm0.72}}$&	${85.17{\scriptsize\pm0.74}}$&	$39.32{\scriptsize\pm0.47}$&	$71.06{\scriptsize\pm0.63}$ \\
& ZOC\cite{zoc}+\textbf{FT}	&	$$ &	$$ &$$&	$$&	$$&	$$&	$2$  \\
&\textbf{ANP+FT}  &	$\mathbf{60.82{\scriptsize\pm1.04}}$ &	${93.20{\scriptsize\pm0.48}}$ &	$\mathbf{95.76{\scriptsize\pm0.16}}$&	$\mathbf{73.86{\scriptsize\pm1.23}}$&	$\mathbf{92.21{\scriptsize\pm1.03}}$&	$\mathbf{54.50{\scriptsize\pm0.44}}$&	$\mathbf{78.39{\scriptsize\pm0.73}}$ \\
\hline
\multirow{2}{*}{\parbox{2cm}{\centering ViT-H-14 OpenCLIP}} & \textbf{ANP}	&$60.14{\scriptsize\pm1.17}$&	${90.98{\scriptsize\pm0.58}}$&	$91.90{\scriptsize\pm0.5}$&	$81.00{\scriptsize\pm0.94}$&	$73.33{\scriptsize\pm1.39}$&	$49.12{\scriptsize\pm1.17}$&	
$74.42{\scriptsize\pm0.96}$ \\
& \textbf{FT}&	$56.10{\scriptsize\pm1.21}$&	$88.30{\scriptsize\pm0.66}$&	$97.78{\scriptsize\pm0.11}$&	$84.83{\scriptsize\pm0.50}$&	$95.96{\scriptsize\pm0.16}$&	$43.25{\scriptsize\pm0.51}$&	$77.71{\scriptsize\pm0.53}$ \\
& \textbf{ANP+FT}	&$\mathbf{64.08{\scriptsize\pm1.12}}$&	$\mathbf{94.06{\scriptsize\pm0.48}}$&	$\mathbf{97.83{\scriptsize\pm0.11}}$&	$\mathbf{87.09{\scriptsize\pm0.61}}$&	$\mathbf{98.15{\scriptsize\pm0.12}}$&	$\mathbf{60.74{\scriptsize\pm0.67}}$&	$\mathbf{83.66{\scriptsize\pm0.52}}$ \\
\bottomrule
\end{tabular}}
\end{table}


% \begin{table}
%   \caption{Average performance for multiple datasets.
%   }
%    \label{tab:main_performance}
%   \centering
%   \scalebox{0.65}{\begin{tabular}{@{}cc|c|c|c||c|c|c||c|c|c@{}}
%     \cline{3-11} %\hline % cmidrule(r){2-5}
%  && \multicolumn{3}{c}{ANPS} & \multicolumn{3}{c}{FT} & \multicolumn{3}{c}{CLIPN} \\
%   \cline{3-11}
%  && Acc & F1 & AUC & Acc & F1 & AUC & Acc & F1 & AUC \\
%     \hline %\hline % cmidrule(r){2-5}
% \multirow{7}{*}{\rotatebox{90}{ViT-B-16}}& inaturalist &	$65.31\pm0.84$ &	$60.82\pm1.04$ &	$73.56\pm1.15$ &	$60.56\pm0.81$ &	$54.39\pm1.02$ &	$68.58\pm1.18$ &	$51.99\pm0.27$ &	$37.94\pm0.46$ &	$65.57\pm1.34$ \\
% & dtd &	$75.58\pm1.06$ &	$73.86\pm1.23$ &	$81.53\pm1.30$ &	$74.18\pm0.91$ &	$73.15\pm1.01$ &	$81.44\pm1.03$ &	$56.21\pm0.31$ &	$45.88\pm0.51$ &	$80.36\pm0.92$ \\
% & eurosat &	$59.74\pm0.37$ &	$54.50\pm0.44$ &	$82.03\pm0.74$ &	$52.37\pm0.38$ &	$42.19\pm0.32$ &	$76.39\pm1.15$ &	$49.81\pm0.25$ &	$35.06\pm0.22$ &	$77.83\pm1.56$ \\
% & food101 &	$95.77\pm0.16$ &	$95.76\pm0.16$ &	$99.16\pm0.06$ &	$94.19\pm0.19$ &	$94.16\pm0.19$ &	$99.20\pm0.06$ &	$61.04\pm0.49$ &	$52.92\pm0.76$ &	$98.73\pm0.07$ \\
% & Pets &	$92.33\pm1.00$ &	$92.21\pm1.03$ &	$95.66\pm1.04$ &	$91.95\pm0.36$ &	$91.80\pm0.39$ &	$98.74\pm0.18$ &	$67.17\pm0.55$ &	$61.96\pm0.82$ &	$96.37\pm0.82$ \\
% & sun397 &	$93.40\pm0.43$ &	$93.20\pm0.48$ &	$98.86\pm0.15$ &	$89.60\pm0.54$ &	$89.17\pm0.60$ &	$98.68\pm0.11$ &	$90.62\pm0.28$ &	$90.49\pm0.29$ &	$98.70\pm0.11$ \\
% \cline{2-11}
% & average &	$80,35\pm0,64$ & $78,39\pm0,73$ &	$88,46\pm0,74$	& $77,14\pm0,53$ & $74,14\pm0,59$ &	$87,17\pm0,62$	& $62,80\pm0,36$ &	$54,04\pm0,51$	& $86,26\pm0,80$ \\
% \hline
% \multirow{7}{*}{\rotatebox{90}{Open-CLIP}}& inaturalist &	$65.31\pm0.84$ &	$60.82\pm1.04$ &	$73.56\pm1.15$ &	$60.56\pm0.81$ &	$54.39\pm1.02$ &	$68.58\pm1.18$ &	$51.99\pm0.27$ &	$37.94\pm0.46$ &	$65.57\pm1.34$ \\
% & dtd &	$75.58\pm1.06$ &	$73.86\pm1.23$ &	$81.53\pm1.30$ &	$74.18\pm0.91$ &	$73.15\pm1.01$ &	$81.44\pm1.03$ &	$56.21\pm0.31$ &	$45.88\pm0.51$ &	$80.36\pm0.92$ \\
% & eurosat &	$59.74\pm0.37$ &	$54.50\pm0.44$ &	$82.03\pm0.74$ &	$52.37\pm0.38$ &	$42.19\pm0.32$ &	$76.39\pm1.15$ &	$49.81\pm0.25$ &	$35.06\pm0.22$ &	$77.83\pm1.56$ \\
% & food101 &	$95.77\pm0.16$ &	$95.76\pm0.16$ &	$99.16\pm0.06$ &	$94.19\pm0.19$ &	$94.16\pm0.19$ &	$99.20\pm0.06$ &	$61.04\pm0.49$ &	$52.92\pm0.76$ &	$98.73\pm0.07$ \\
% & Pets &	$92.33\pm1.00$ &	$92.21\pm1.03$ &	$95.66\pm1.04$ &	$91.95\pm0.36$ &	$91.80\pm0.39$ &	$98.74\pm0.18$ &	$67.17\pm0.55$ &	$61.96\pm0.82$ &	$96.37\pm0.82$ \\
% & sun397 &	$93.40\pm0.43$ &	$93.20\pm0.48$ &	$98.86\pm0.15$ &	$89.60\pm0.54$ &	$89.17\pm0.60$ &	$98.68\pm0.11$ &	$90.62\pm0.28$ &	$90.49\pm0.29$ &	$98.70\pm0.11$ \\
% \cline{2-11}
% & average &	$80,35\pm0,64$ & $78,39\pm0,73$ &	$88,46\pm0,74$	& $77,14\pm0,53$ & $74,14\pm0,59$ &	$87,17\pm0,62$	& $62,80\pm0,36$ &	$54,04\pm0,51$	& $86,26\pm0,80$ \\
% \hline
% \end{tabular}}
 
% \end{table}

